Provably Total Functions of Arithmetic with Basic Terms

A new characterization of provably recursive functions of first-order arithmetic is described. Its main feature is using only terms consisting of 0, the successor S and variables in the quantifier rules, namely, universal elimination and existential introduction.

==> eptcsdata.tex <==
\providecommand{\firstpage}{28}
\providecommand{\publicationstatus}{Jean-Yves Marion (Ed.): Second Workshop on\\
Developments in Implicit Computational Complexity (DICE 2011) \\
EPTCS 75, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.75.3}{10.4204/EPTCS.75.3}}
\pdfoutput=1

